Systematic Mutation-based Evaluation of the Soundness of Security-focused Android Static Analysis Techniques

Mobile application security has been a major area of focus for security research over the course of the last decade. Numerous application analysis tools have been proposed in response to malicious, curious, or vulnerable apps. However, existing tools, and specifically, static analysis tools, trade soundness of the analysis for precision and performance and are hence soundy. Unfortunately, the specific unsound choices or flaws in the design of these tools is often not known or well-documented, leading to misplaced confidence among researchers, developers, and users. This paper describes the Mutation-based Soundness Evaluation ($\mu$SE) framework, which systematically evaluates Android static analysis tools to discover, document, and fix flaws, by leveraging the well-founded practice of mutation analysis. We implemented $\mu$SE and applied it to a set of prominent Android static analysis tools that detect private data leaks in apps. In a study conducted previously, we used $\mu$SE to discover $13$ previously undocumented flaws in FlowDroid, one of the most prominent data leak detectors for Android apps. Moreover, we discovered that flaws also propagated to other tools that build upon the design or implementation of FlowDroid or its components. This paper substantially extends our $\mu$SE framework and offers an new in-depth analysis of two more major tools in our 2020 study, we find $12$ new, undocumented flaws and demonstrate that all $25$ flaws are found in more than one tool, regardless of any inheritance-relation among the tools. Our results motivate the need for systematic discovery and documentation of unsound choices in soundy tools and demonstrate the opportunities in leveraging mutation testing in achieving this goal.

==> bib/__latexindent_temp.tex <==

@online{android-fragments,
	title = {{Fragments | Android Developers}},
    author={Android Developers},
    url= {https://developer.android.com/guide/components/fragments.html},
    year={2019}
    }

@MISC{activitylauncher,
  AUTHOR = {{F-Droid}},
  TITLE = {{Activity Launcher}},
  HOWPUBLISHED = {\url{https://f-droid.org/packages/de.szalkowski.activitylauncher/}},
}

@online{fdroid_release,
	title = {{FlowDroid 2.0}},
    author={Steven Artz},
    url= {https://github.com/secure-software-engineering/soot-infoflow/releases},
    year={2019}
    }

@MISC{fdroid_git,
  AUTHOR = {{stream101}},
  TITLE = {{Possible to integrate Fragment lifecycle ?}},
  HOWPUBLISHED = {\url{https://github.com/secure-software-engineering/soot-infoflow-android/issues/52}},
}

@MISC{nogotofail,
  AUTHOR = {{Google}},
  TITLE = {{nogotofail}},
  HOWPUBLISHED = {\url{https://github.com/google/nogotofail}},
}

@MISC{android-work,
  AUTHOR = {{Android}},
  TITLE = {{Android for Work}},
  HOWPUBLISHED = {\url{https://www.android.com/work/}},
}

@MISC{provider-basics,
  AUTHOR = {{Android Developers}},
  TITLE = {{Content Provider Basics}},
  HOWPUBLISHED = {\url{https://developer.android.com/guide/topics/providers/content-provider-basics.html}},
}

@MISC{knox,
  AUTHOR = {{Samsung Electronics}},
  TITLE = {{An Overview of Samsung Knox}},
  HOWPUBLISHED = {\url{http://www.samsung.com/global/business/business-images/resource/white-paper/2014/02/Samsung_KNOX_whitepaper_June-0-0.pdf}},
  YEAR = 2013,
}

@MISC{tasks,
  AUTHOR = {{Android Developers }},
  TITLE = {{Tasks and Back Stack}},
  HOWPUBLISHED = {\url{https://developer.android.com/guide/components/tasks-and-back-stack.html}},
}

@MISC{google-play-apps,
  AUTHOR = {{Statista}},
  TITLE = {{Number of available applications in the Google Play Store from December 2009 to February 2016}},
  HOWPUBLISHED = {\url{http://www.statista.com/statistics/266210/number-of-available-applications-in-the-google-play-store/}},
}

@MISC{k9,
  AUTHOR={K-9 Mail developers},
  TITLE={{K-9 Mail}},
  HOWPUBLISHED={\url{https://github.com/k9mail}},
  YEAR=2015,
}

@MISC{total-apps-statista,
  AUTHOR = {{The Statista Portal}},
  TITLE = {{Number of apps available in leading app stores as of March 2017}},
  HOWPUBLISHED = {\url{https://www.statista.com/statistics/276623/number-of-apps-available-in-leading-app-stores/}},
}

@MISC{economist,
  AUTHOR = {The Economist},
  TITLE = {{Planet of the phones}},
  HOWPUBLISHED = {\url{http://www.economist.com/news/leaders/21645180-smartphone-ubiquitous-addictive-and-transformative-planet-phones}},
  MONTH = feb,
  YEAR = 2015,
}

@MISC{smith15,
  AUTHOR = {Aaron Smith},
  TITLE = {{U.S. Smartphone Use in 2015}},
  HOWPUBLISHED = {\url{http://www.pewinternet.org/2015/04/01/us-smartphone-use-in-2015/}},
  MONTH = apr,
  YEAR = 2015,
}

@MISC{expensivewall,
  AUTHOR = {Elena Root and Andrey Polkovnichenko and Bohdan Melnykov},
  TITLE = {{ExpensiveWall: A dangerous ‘packed’ malware on Google Play that will hit your wallet}},
  HOWPUBLISHED = {\url{https://blog.checkpoint.com/2017/09/14/expensivewall-dangerous-packed-malware-google-play-will-hit-wallet/}},
  MONTH = Aug,
  YEAR = 2017,
}

@MISC{badtrustmanager,
  AUTHOR = {{Nilanchala}},
  TITLE = {{How to Trust All Certificates for HttpURLConnection in Android}},
  HOWPUBLISHED = {\url{http://stacktips.com/snippet/how-to-trust-all-certificates-for-httpurlconnection-in-android}},
  NOTE = {Last accessed on November 5, 2017}
    
}


@online{android-adt-obsolete,
    AUTHOR = {{Android Developers}},
    lastaccessed ={July 7, 2019},
    TITLE = {{An update on Eclipse Android Developer Tools}},
    year =  "2019",
    url =  {https://android-developers.googleblog.com/2015/06/an-update-on-eclipse-android-developer.html}
    
}

==> discussion.tex <==
\vspace{-0.3em}
\section{Discussion and Conclusion}
\label{sec:discussion}
\vspace{-0.2em}

Designing \detectors is in no way a simple task; tool designers have to balance several orthogonal requirements such as detecting as many vulnerabilities as possible without introducing false positives, while also scaling to large codebases. %
Yet, the fact remains that there is significant room for improvement in how \detectors are built and evaluated, as evidenced by the flaws discovered by \tool.

To move forward, we need to understand the divergent perspectives regarding the design of \detectors, and reach a consensus (or at least an agreeable minima) in terms of what is expected from \detectors and how we will design and evaluate them to satisfy the expectations.%
We seek to begin this discourse within the security community through a discussion that integrates several views on the design decisions behind \detectors, informed by our results and conversations with tool designers during the vulnerability reporting process.%






\vspace{-0.3em}
\subsection{Security-centric Evaluation vs. Technique-centric Design}
\vspace{-0.2em}
Determining what misuse is within or outside the scope for a \detector is a complex question that yields several different viewpoints.
This paper's view is {\em security-centric}, \ie even if some misuse instances may seem unlikely or evasive, \detectors that target security-focused use cases (\eg compliance, auditing) should attempt to account for them.
However, we observe that tool designers typically adhere to a {\em technique-centric} perspective, \ie the design of \detectors is not influenced by a threat model, but mainly by what static analysis can and cannot accomplish (while implicitly assuming a benign developer).
This quote from the maintainers of \cryptoguard highlights this view, wherein they state that the ``lines'' between what is within/outside scope \emphdblquote{seen so far were technically motivated -- not use-case motivated..should we use alias analysis?...}.
This gap in perspective does not mean that \detectors may not detect any of the mutants generated by \tool using operators based on the \ref{adversary:evasive} threat model; rather, it only means that detection (or lack thereof) may not be {\em caused} by a security-centric design.

\subsection{Defining ``Scope'' for the Technique-centric Design}
\label{sec:discussion-within-scope}
We observe that even within \detectors that take a \textit{technique-centric} approach, there is little agreement on the appropriate scope of detection.
For instance, \xanitizer focuses on catching every possible misuse instance, regardless of any external factors such as whether that kind of misuse is observed in the wild, or a threat model, as the designers believe that \emphdblquote{the distinction should not be between `common' and `uncommon', but instead between `can be (easily) computed statically' and `can not be computed'.}.
This may also result in \xanitizer not detecting a commonly observed misuse that is difficult to compute statically, although we did not observe such cases.%

In contrast, \cryptoguard, \cognicrypt, \codeqlgcs/\codeqllgtm (same developers), and \spotbug would {\em consider seemingly-unlikely/evasive flaws} {\em within scope} (\eg\ \fnumber{3}$\rightarrow$\fnumber{6}, \fnumber{8}), because they were found in the wild (unlike \xanitizer, for which this is not a consideration); \eg as stated by \spotbug maintainers, \emphdblquote{Any code pattern seen in a real code base will likely be considered.}.
This view aligns with our perspective, that regardless of how the mutants were generated, if a misuse instance (representing a flaw) is discovered in real apps (which is {\em true for all flaws except \fnumber{12} and \fnumber{13}}, it should be within the detection scope.
However, \spotbug, \codeqlgcs, and \codeqllgtm maintainers extend this definition with the condition that the observations in the wild be frequent to motivate change.
These divergent design perspectives motivate the need to clearly define the expectations from \detectors.





\subsection{Utility of Seemingly-Uncommon or Evasive Tests}
\label{sec:discussion-evasive}
As the designers of \coverity state from practical deployment experience in 2010~\cite{BBC+10}, \emphdblquote{No bug is too foolish to check for}, and that \emphdblquote{Given enough code, developers will write almost anything you can think of...}.
The results from our evaluation and the impact study corroborate this sentiment, \ie\ \fnumber{3}$\rightarrow$\fnumber{6} and \fnumber{8} were all obtained using operators (\opnumber{3}, \opnumber{4}, and \opnumber{6}) modeled to emulate threats \ref{adversary:benign_accident} and \ref{adversary:benign_fixing}, \ie representing {\em benign} behavior (however unlikely); and indeed, these flaws were later found in supposedly benign applications.
This suggests that the experience of the \coverity designers is valid a decade later, making it important to evaluate \detectors with ``more-than-trivial'' cases to not only test their detection prowess, but to also account for real problems that may exist in the wild.





\subsection{The Need to Strengthen Crypto-Detectors}
\label{sec:discussion-need-stronger}
We argue that it is not only justified for tools to detect uncommon cases (\eg given that even benign developers write seemingly-unlikely code), but also critical for their sustained relevance.
As the designers of \coverity found~\cite{BBC+10}, false negatives matter from a commercial perspective, because \emphdblquote{Potential customers intentionally introduced bugs into the system, asking {`Why didn't you find it?'}}.

Perhaps more significantly, the importance of automated \detectors with the ability to guarantee {\em assurance} is significantly rising with the advent of new {\em compliance} legislation such as the IoT Cybersecurity Improvement Act of 2020~\cite{iot-bill}, which seeks to rein in vulnerabilities in billions of IoT systems that include vulnerable server-side/mobile components.
Vulnerabilities found {\em after} a compliance certification may result in penalties for the offending IoT developers, and financial consequences for the compliance checkers/labs and \detectors used. %
Complementing static detection with manual or dynamic analysis may be infeasible at this scale, as tool designers noted:
\eg\ \emphdblquote{...review an entire codebase at once, manual review can be difficult.} (\codeqllgtm) and \emphdblquote{Existing dynamic analysis tools will be able to detect them only if the code is triggered (which can be notoriously difficult)} (\cryptoguard).
Thus, static \detectors will need to become more robust, and capable of detecting hard-to-detect misuse instances.





\subsection{Towards Crypto-Detectors Strengthened by a Security-Centric Evaluation}
\label{sec:evolution-conclusion}

Fortunately, we observe that there is support among tool designers for moving towards stronger security guarantees. %
 For instance, \cognicrypt designers encourage the possibility of expressing evasive scenarios in the \crysl language, and state that \ie \emphdblquote{...what would be a nice future direction is to tweak the SAST with such optimizations/ more analysis but still allow the \crysl developer to decide if he wants to switch these `evasive user' checks...},
% {\color{blue}
but indicate the caveat that developers may not use such additional configuration options~\cite{JSMB13}.
However, we believe that such options will benefit {\em independent evaluators}, as well as developers who are unsure of the quality of their own supply chain, to perform a hostile review of the third-party code at their disposal.
% }
Similarly, the \cryptoguard designers state that \emphdblquote{...this insight of evasive developers is very interesting and timely, which immediately opens up new directions.}
This potential paradigm-shift towards a {\em security-focused} design of \detectors is timely, and
\tool's rigorous evaluation with expressive test cases can play an effective role in it, by enabling tool designers to proactively address gaps in detection during the design phase itself, rather than reactively (\ie after a vulnerability is discovered in the wild).
More importantly, further large-scale evaluations using \tool, and the flaws discovered therein, will enable the community to continually examine the design choices made by \detectors and reach consensus on what assurances we can feasibly expect. %
We envision that such development aided by \tool will lead to a mature ecosystem of \detectors with a well-defined and strong security posture, and which can hold their own in adversarial situations (\eg compliance assessments) within certain {\em known} bounds, which will eventually lead to long-lasting security benefits for end-user software.


==> tables/tool_table2.tex <==
\begin{table}
    \scriptsize
    \centering
    \caption{{\small The number and percentage of leaks not detected by $3$
    popular data leak detection tools.  }}
    \label{tbl:tool_table}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{c|c|c}
      \Xhline{2\arrayrulewidth}
      {\bf Tool}	& {\bf Undetected Leaks} & {\bf
      Undetected Leaks (\%)} \\
      \Xhline{2\arrayrulewidth}
      FlowDroid v2.0 & 987$/$2,026  & 48.7\% \\
      Argus & 1,480$/$2,026  &  73.1\%\\
      DroidSafe & 83$/$2,026  & 4.1\% \\
      \Xhline{2\arrayrulewidth}
    \end{tabular} 
    % \vspace{-2em}
    \end{table}
    
    

==> texfiles/argus_vulnerability.tex <==
\input{tables/vuln_table_argus.tex}

\subsubsection{Argus Analysis}\label{sec:argus_vuln}
\add{
Through this experiment, we analyzed Argus for \soundiness{} issues, following
the methodology described in Section~\ref{sec_tool_analysis}.
We choose Argus for two reasons: {\sf (1)} impact (Argus is cited by 200+ papers), and
{\sf (2)} potential for change, as it is being actively maintained by its
authors.}

\myparagraph{Results} We discovered \(9\) unique flaws of Argus,
\textit{separate from} the ones found from FlowDroid analysis as described in
Section~\ref{sec:flowdroid_vuln}. We provide the result of \tools{} analysis for
Argus in Table~\ref{tab:argus-vuln-descs}. We have additionally reported these
flaws to the authors of Argus to resolve the issues.

Of the \(9\) issues, \(4\) issues are based on Fragment usage and are of FC1
flaw class. In FlowDroid study, we already found using \tool{} that fragment
based leaks are not detected well in FlowDroid. During Argus analysis,
we look at fragments in-depth using \tool{} to find these flaws in Argus. Next,
we discuss the nature of flaws we found in Argus.

\myparagraph{Variants of Fragment based Flaws} To ensure that our findings are
reproducible and authentic, we prepare minimal Android applications which
contain flaws (available in our accompanying
repository~\cite{appendix}). The general structure of the application contains a
single activity and a single fragment within the activity class. For minimal
interaction, button type widgets are introduced within the fragment. Event
listening methods are defined within the Activity class, and fragment \(XML\)
file is used to couple the event listening methods with the corresponding
widgets. The event listening methods when used may introduce leak source to a
field variable. The details of each fragment variant are provided in
Table~\ref{tab:argus-vuln-descs}. These flaws can be categorized as of FC1:
Missing callbacks due to the event driven nature.

\myparagraph{Variants of \recycler{} Widget based Flaws}
The remaining \(5\) flaws we found in Argus are based on \recycler{} widgets.
\recycler{} is an established widget from default SDK of Android, and is used to
show a collection of data within a limited, scrolling window. Each \recycler{}
widget implementation requires implementing classes extending
\recyclerviewholder{} and \recycleradapter{}. Moreover, these classes contain
several abstract methods which are required to be implemented to function
properly, namely {\sf onCreateViewHolder}, {\sf onBindViewHolder} and {\sf
getItemCount}. Through our experiment, we observed that leaks placed at these
components in those methods are not detected {\em at all} in Argus. Summary of
these flaws are tabulated in Table~\ref{tab:argus-vuln-descs}, and the example
minimal Android minimal APKs, each exhibiting a single flaw are
available in~\cite{appendix}. All the flaws of this particular class can be
categorized as FC2: Missing Implicit calls.

==> texfiles/flowdroid_vuln.tex <==
\subsubsection{FlowDroid Analysis}\label{sec:flowdroid_vuln}
\input{tables/vuln_table}
This experiment demonstrates an in-depth, manual analysis of FlowDroid v2.0,
which was available when we started this study. As mentioned earlier, we chose
it due to its potential for change and for its impact (700+ citations).

\myparagraph{Results} We discovered $13$ unique flaws, from FlowDroid alone,
demonstrating that \tool can be effectively used to find problems that can be
resolved to flaws (\ref{rq:findings}).  Using the approach from
Section~\ref{sec:feasibility}, the analyst
needed less than an hour to isolate a flaw from the set of undetected mutants,
in the worst case.  In the best case, flaws were found in a matter of minutes,
demonstrating that the amount of manual effort required to quickly find flaws
using \tool{} is minimal (\ref{rq:feasible}).  We give descriptions of the flaws
discovered as a result of \tools{} analysis in
\autoref{tab:flowdroid-vuln-descs}.

We have reported these flaws and are working with the developers to resolve the
issues. In fact, we developed patches to correctly implement Fragment support
(\ie{} flaw \(13\) in Table~\ref{tab:flowdroid-vuln-descs}), which were accepted
by developers.
To gain insight about the practical challenges faced by static analysis tools,
and their design flaws, we further categorize the discovered flaws into the
following {\em flaw classes}:

\myparagraph{FC1: Missing Callbacks} The security tool (\eg, FlowDroid) does not
recognize some callback method(s), and will not find leaks placed within them.
Tools that use lists of APIs or callbacks are susceptible to this problem, as
prior work has demonstrated as the generated list of callbacks {\sf (1)} may not
be complete, and {\sf (2)} or may not be updated as the Android platform
evolves.
%{\color{blue}
We found both these cases in our analysis of FlowDroid. That is, {\sf
DialogFragments} was added in API 11, \ie, {\em before FlowDroid was released},
and {\sf NavigationView} was added after.  These limitations are well-known in
the community of researchers at the intersection of program analysis and Android
security and have been documented by prior work~\cite{cfb+15}.  However, \tool
helps evaluate the robustness of existing security tools against these flaws,
and helps in uncovering these undocumented flaws for the wider security
audience.  Additionally, {\em some of these flaws may not be resolved even after
adding the callback to the list}; \eg, {\sf PhoneStateListener} and {\sf
SQLiteOpenHelper}, both added in API 1, are not interfaces, but abstract
classes. Therefore, adding them to FlowDroid's list of callbacks (\ie, {\sf
AndroidCallbacks.txt}) does not resolve the issue.
%}

\myparagraph{FC2: Missing Implicit Call} The security tool does not identify
leaks within some method that is implicitly called by another method.  For
instance, FlowDroid does not recognize the path to {\sf Runnable.run()} when a
Runnable is passed into the {\sf ExecutorService.submit(Runnable)}. The response
from the developers indicated that this class of flaws was due to an unresolved
design challenge in Soot's~\cite{vcg+99} SPARK algorithm, upon which FlowDroid
depends.
%{\color{blue}
This limitation is in addition known within the program analysis
community~\cite{cfb+15}. However, the documentation of this gap, thanks to
\tool, would certainly help developers and researchers in the wider security
community.
%}

\myparagraph{FC3: Incorrect Modeling of Anonymous Classes} The security tool
misses data leaks expressed within an anonymous class. For example, FlowDroid
does not recognize leaks in the {\sf onReceive()} callback of a dynamically
registered {\sf BroadcastReceiver}, which is implemented within another
dynamically registered BroadcastReceiver's {\sf onReceive()} callback. It is
important to note that finding such complex flaws is only possible due to
\tool's semi-automated mechanism, and may be rather prohibitive for an entirely
manual analysis.

\myparagraph{FC4: Incorrect Modeling of Asynchronous Methods} The security tool
does not recognize a data leak whose source and sink are called within different
methods that are asynchronously executed. For instance, FlowDroid does not
recognize the flow between data leaks in two callbacks (\ie, {\sf
onLocationChanged} and {\sf onStatusChanged}) of the {\sf LocationListener}
class, which the adversary may cause to execute sequentially (\ie, as our EE
confirmed).

Apart from {\bf FC1}, which may be patched with limited efforts, the other three
categories of flaws may require a significant amount of research effort to
resolve. However, documenting them is critical to increase awareness of real
challenges faced by Android static analysis tools.

\add{During this study, FlowDroid 2.0 became unavailable \ie{} after we
had communicated the initial flaws discovered in 7 apps, but before we added the
additional 8 apps. Therefore, we continued with
the then available versions of FlowDroid from v\(2.5\) to v\(2.7.1\) for the
later parts of study.}

==> texfiles/performance_analysis.tex <==
\section{Performance Analysis of Execution Engine}
